Higgs production and decay with a fourth Standard-Model-like fermion generation

State-of-the-art predictions for the Higgs-boson production cross section via gluon fusion and for all relevant Higgs-boson decay channels are presented in the presence of a fourth Standard-Model-like fermion generation. The qualitative features of the most important differences to the genuine Standard Model are pointed out, and the use of the available tools for the predictions is described. For a generic mass scale of 400-600 GeV in the fourth generation explicit numerical results for the cross section and decay widths are presented, revealing extremely large electroweak radiative corrections, e.g., to the cross section and the Higgs decay into WW or ZZ pairs, where they amount to about -50% or more. This signals the onset of a non-perturbative regime due to the large Yukawa couplings in the fourth generation. An estimate of the respective large theoretical uncertainties is presented as well.

==> plots/BR_gaga_scan.tex <==
\begin{table}
\begin{center}
\caption[]{\label{tab:EWNLOBRGG}{Higgs branching fractions for the $\PGg\PGg$ decay channel without
    and with NLO EW corrections.}}  \vspace{1em}
\begin{tabular}{|ccc|}
\hline
\rule[-1ex]{0ex}{3.5ex}%
$\MH\,$[GeV] &
w/o NLO EW       &
w/ NLO EW           \\
\hline
\rule[0ex]{0ex}{2.5ex}%
$100$ & $1.52\,\cdot\,10^{-4}$  & $8.90\,\cdot\,10^{-7}$ \\
$110$ & $1.97\,\cdot\,10^{-4}$  & $3.45\,\cdot\,10^{-6}$ \\
$120$ & $2.52\,\cdot\,10^{-4}$  & $9.32\,\cdot\,10^{-6}$ \\
$130$ & $3.13\,\cdot\,10^{-4}$  & $2.08\,\cdot\,10^{-5}$ \\
$140$ & $3.73\,\cdot\,10^{-4}$  & $4.03\,\cdot\,10^{-5}$ \\
$150$ & $4.05\,\cdot\,10^{-4}$  & $6.83\,\cdot\,10^{-5}$%
\rule[-1ex]{0ex}{2.5ex}\\
\hline
\end{tabular}
\end{center}
\end{table}


==> plots/ggf_8tev.tex <==
\tabcolsep 4pt
\begin{tabular}{cccc}
\hline
\rule[-1ex]{0ex}{3.5ex}%
$\MH$ [GeV] & $\Mbp$ [GeV] & $\Mnp$ [GeV] & $\sigma$ [pb] &
\hline
\rule[-0ex]{0ex}{2.5ex}%

 120  &   450  &   350  &        199.6  \\
 120  &   450  &   375  &        199.9  \\
 120  &   450  &   400  &        200.3  \\
 120  &   500  &   350  &        199.2  \\
 120  &   500  &   375  &        199.6  \\
 120  &   500  &   400  &        200.0  \\  
 120  &   550  &   350  &        199.3  \\
 120  &   550  &   375  &        199.7  \\
 120  &   550  &   400  &        200.1  \\

 350  &   450  &   350  &        9.940  \\
 350  &   450  &   375  &        9.961  \\
 350  &   450  &   400  &        9.986  \\
 350  &   500  &   350  &        9.901  \\
 350  &   500  &   375  &        9.922  \\
 350  &   500  &   400  &        9.946  \\
 350  &   550  &   350  &        9.899  \\
 350  &   550  &   375  &        9.920  \\
 350  &   550  &   400  &        9.944  \\

 600  &   450  &   300  &        1.236  \\
 600  &   450  &   350  &        1.280  \\
 600  &   450  &   400  &        1.292  \\
 600  &   500  &   300  &        1.209  \\
 600  &   500  &   350  &        1.253  \\
 600  &   500  &   400  &        1.271  \\
 600  &   550  &   300  &        1.193  \\
 600  &   550  &   350  &        1.236  \\
 600  &   550  &   400  &        1.248  \\

                                                                            1,1           Top












100 & 244  & 200 & 48.6    \\ 
110 & 199  & 250 & 27.7    \\
120 & 165  & 300 & 17.6    \\ 
130 & 138  & 400 & 9.59    \\
140 & 117  & 500  & 3.70   \\
150 & 99.2 & 600  & 1.40   \\
160 & 84.5 & 700  & 0.556  \\
170 & 73.0  & & 800  & 0.235  \\
180 & 63.1 & 900  & 0.104  \\
190 & 55.2 & 1000 & 0.0  & 456%
\rule[-1ex]{0ex}{2.5ex}\\
\hline
\end{tabular}


==> plots/ggf_grid_8tev.tex <==
\tabcolsep 4pt
\begin{tabular}{|cccc|}
\hline
\rule[-1ex]{0ex}{3.5ex}%
$\MH$ [GeV] & $\Mbp$ [GeV] & $\Mnp$ [GeV] & $\sigma$ [pb] \\
\hline
\rule[-0ex]{0ex}{2.5ex}%
 120  &   450  &   350  &        199.6  \\
 120  &   450  &   375  &        199.9  \\
 120  &   450  &   400  &        200.3  \\
 120  &   500  &   350  &        199.2  \\
 120  &   500  &   375  &        199.6  \\
 120  &   500  &   400  &        200.0  \\  
 120  &   550  &   350  &        199.3  \\
 120  &   550  &   375  &        199.7  \\
 120  &   550  &   400  &        200.1  \\

 350  &   450  &   350  &        9.940  \\
 350  &   450  &   375  &        9.961  \\
 350  &   450  &   400  &        9.986  \\
 350  &   500  &   350  &        9.901  \\
 350  &   500  &   375  &        9.922  \\
 350  &   500  &   400  &        9.946  \\
 350  &   550  &   350  &        9.899  \\
 350  &   550  &   375  &        9.920  \\
 350  &   550  &   400  &        9.944  \\

 600  &   450  &   300  &        1.236  \\
 600  &   450  &   350  &        1.280  \\
 600  &   450  &   400  &        1.292  \\
 600  &   500  &   300  &        1.209  \\
 600  &   500  &   350  &        1.253  \\
 600  &   500  &   400  &        1.271  \\
 600  &   550  &   300  &        1.193  \\
 600  &   550  &   350  &        1.236  \\
 600  &   550  &   400  &        1.248  \\
\rule[-1ex]{0ex}{2.5ex}\\
\hline
\end{tabular}

